Hardware/Software Co-Assurance using the Rust Programming Language and ACL2

The Rust programming language has garnered significant interest and use as a modern, type-safe, memory-safe, and potentially formally analyzable programming language. Our interest in Rust stems from its potential as a hardware/software co-assurance language, with application to critical systems such as autonomous vehicles. We report on the first known use of Rust as a High-Level Synthesis (HLS) language. Most incumbent HLS languages are a subset of C. A Rust-based HLS brings a single modern, type-safe, and memory-safe expression language for both hardware and software realizations with high assurance. As a a study of the suitability of Rust as an HLS, we have crafted a Rust subset, inspired by Russinoff's Restricted Algorithmic C (RAC), which we have imaginatively named Restricted Algorithmic Rust, or RAR. In our first implementation of a RAR toolchain, we simply transpile the RAR source into RAC. By so doing, we leverage a number of existing hardware/software co-assurance tools with a minimum investment of time and effort. In this paper, we describe the RAR Rust subset, detail our prototype RAR toolchain, and describe the implementation and verification of several representative algorithms and data structures written in RAR, with proofs of correctness conducted using the ACL2 theorem prover.

==> eptcsdata.tex <==
\providecommand{\firstpage}{202}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.16}{10.4204/EPTCS.359.16}}
\pdfoutput=1

